Parallel Batch-Dynamic $k$-Clique Counting

In this paper, we study new batch-dynamic algorithms for the $k$-clique counting problem, which are dynamic algorithms where the updates are batches of edge insertions and deletions. We study this problem in the parallel setting, where the goal is to obtain algorithms with low (polylogarithmic) depth. Our first result is a new parallel batch-dynamic triangle counting algorithm with $O(\Delta\sqrt{\Delta+m})$ amortized work and $O(\log^* (\Delta+m))$ depth with high probability, and $O(\Delta+m)$ space for a batch of $\Delta$ edge insertions or deletions. Our second result is an algebraic algorithm based on parallel fast matrix multiplication. Assuming that a parallel fast matrix multiplication algorithm exists with parallel matrix multiplication constant $\omega_p$, the same algorithm solves dynamic $k$-clique counting with $O\left(\min\left(\Delta m^{\frac{(2k - 1)\omega_p}{3(\omega_p + 1)}}, (\Delta+m)^{\frac{2(k + 1)\omega_p}{3(\omega_p + 1)}}\right)\right)$ amortized work and $O(\log (\Delta+m))$ depth with high probability, and $O\left((\Delta+m)^{\frac{2(k + 1)\omega_p}{3(\omega_p + 1)}}\right)$ space. Using a recently developed parallel $k$-clique counting algorithm, we also obtain a simple batch-dynamic algorithm for $k$-clique counting on graphs with arboricity $\alpha$ running in $O(\Delta(m+\Delta)\alpha^{k-4})$ expected work and $O(\log^{k-2} n)$ depth with high probability, and $O(m + \Delta)$ space. Finally, we present a multicore CPU implementation of our parallel batch-dynamic triangle counting algorithm. On a 72-core machine with two-way hyper-threading, our implementation achieves 36.54--74.73x parallel speedup, and in certain cases achieves significant speedups over existing parallel algorithms for the problem, which are not theoretically-efficient.

==> experiment-figures.tex <==
\onecolumn
\begin{figure}
  \centering
      \includegraphics[width=0.8\textwidth]{figs/speed-up.pdf}
  \caption{Parallel speedup of our batch-dynamic triangle counting algorithm
  with respect to thread count on the Orkut graph. ``144'' indicates 72 cores with hyper-threading. The experiment is
  run with a batch size of $2\times 10^{5}$. }\label{fig:speed-up}
\end{figure}

\begin{figure}
  \centering
      \includegraphics[width=0.8\textwidth]{figs/makkar}
  \caption{Comparison of the performance of our implementation (DLSY, solid line) and  Makkar et al. algorithm~\cite{Makkar2017} (makkar, dotted line).
The figure shows the average batch time for different batch sizes on the rMAT graph with different number of edges sampled. The number of unique edges sampled are shown on the $x$-axis. The number of vertices is fixed at 16,384.
The dark blue, red, green, and light blue lines are for batches of size  $2\times 10^{3}$,  $2\times 10^{4}$,  $2\times 10^{5}$,
and  $2\times 10^{6}$ respectively.
  We see that our new algorithm is faster for small batches and on denser graphs. 
  }\label{fig:makkar}
\end{figure}

\twocolumn

